Exact Certification of (Graph) Neural Networks Against Label Poisoning

Machine learning models are highly vulnerable to label flipping, i.e., the adversarial modification (poisoning) of training labels to compromise performance. Thus, deriving robustness certificates is important to guarantee that test predictions remain unaffected and to understand worst-case robustness behavior. However, for Graph Neural Networks (GNNs), the problem of certifying label flipping has so far been unsolved. We change this by introducing an exact certification method, deriving both sample-wise and collective certificates. Our method leverages the Neural Tangent Kernel (NTK) to capture the training dynamics of wide networks enabling us to reformulate the bilevel optimization problem representing label flipping into a Mixed-Integer Linear Program (MILP). We apply our method to certify a broad range of GNN architectures in node classification tasks. Thereby, concerning the worst-case robustness to label flipping: $(i)$ we establish hierarchies of GNNs on different benchmark graphs; $(ii)$ quantify the effect of architectural choices such as activations, depth and skip-connections; and surprisingly, $(iii)$ uncover a novel phenomenon of the robustness plateauing for intermediate perturbation budgets across all investigated datasets and architectures. While we focus on GNNs, our certificates are applicable to sufficiently wide NNs in general through their NTK. Thus, our work presents the first exact certificate to a poisoning attack ever derived for neural networks, which could be of independent interest. The code is available at https://github.com/saper0/qpcert.

==> sections/02_preliminaries_old.tex <==
\section{Background}
\label{sec:preliminaries}
We consider the task of semi-supervised node classification, where the input graph $\mG = (\mS, \mX)$ contains $n$ nodes, each associated with a feature vector $\vx_i \in \mathbb{R}^d$ collected in the feature matrix $\mX \in \mathbb{R}^{n \times d}$. The graph structure is encoded in the matrix $\mS \in \mathbb{R}_{\ge0}^{n \times n}$, typically representing a type of adjacency matrix. Labels $\rvy\in \{1, \dots, K\}^m$ are provided for a subset of $m$ nodes ($m \le n$). Without loss of generality, we assume that the first $m$ nodes are labeled. The objective is to predict the labels for the remaining $n - m$ unlabeled nodes in a transductive setting or to classify newly added nodes in an inductive setting.  

\textbf{GNNs.} An $L$-layer GNN $f_\theta$ with learnable parameters $\theta$ takes the graph $\mG$ as input and outputs a prediction for each node with $f_\theta(\mG) \in \mathbb{R}^{n \times K}$ for multiclass and  $f_\theta(\mG) \in \mathbb{R}^{n}$ for binary classification; the output for a node $i$ is denoted by $f_\theta(\mathcal{G})_i$. Following \citet{gosch2024provable}, we consider GNNs with a linear output layer parameterized using weights $\mW^{(L+1)}$. Details on the used architectures can be found in \Cref{sec:results}. 

\textbf{Neural Tangent Kernel.} In general, the NTK between two inputs $\rvx_i$ and $\rvx_j$ for a network $f_\theta$ is defined as $\Theta_{ij} = \mathbb{E}_\theta[\linnerprod \nabla_{\theta}f_\theta(\rvx_i),  \nabla_{\theta}f_\theta(\rvx_j) \rinnerprod] \in \mathbb{R}$, where the expectation is taken over the parameter initialization. In a node-classification context, this translates to the NTK being computed between two nodes $i$ and $j$ as $\Theta_{ij} = \mathbb{E}_\theta[\linnerprod \nabla_{\theta}f_\theta(\mG)_i,  \nabla_{\theta}f_\theta(\mG)_j \rinnerprod]$ \citep{sabanayagam2023analysis}. If the width of the network goes to infinity and the parameters are initialized with a Gaussian distribution $\mathcal{N}(0, 1/\text{width})$, the training dynamics are exactly described by the NTK associated to the NN \citep{jacot2018neural, arora2019exact, liu2020linearity}. Specifically, for classification using a soft-margin loss, the training dynamics are equivalent to that of an SVM with the NTK of the NN as its kernel \citep{chen2021equivalence}. This equivalence extends to GNNs \citep{gosch2024provable}.
%Neural networks trained with gradient descent converge to a kernel machine in the infinite width limit, when initialized with parameters from a Gaussian distribution $\mathcal{N}(0, 1/\text{width})$. The training dynamics of these networks are exactly characterized by their NTK counterpart \citep{jacot2018neural, arora2019exact, liu2020linearity}. Specifically, when using a soft-margin loss, the training dynamics of the NN is equivalent to that of an SVM with the NTK corresponding to the NN as the kernel \citep{chen2021equivalence}. This equivalence extends to GNNs as well, as shown in \citet{gosch2024provable}. The NTK between two inputs $\rvx_i$ and $\rvx_j$ of a network $f_\theta(\rvx)$ with parameters $\theta$ is defined as $\Theta_{ij} = \rmQ({\rvx_i,  \rvx_j}) = \mathbb{E}_\theta[\linnerprod \nabla_{\theta}f_\theta(\rvx_i),  \nabla_{\theta}f_\theta(\rvx_j) \rinnerprod] \in \mathbb{R}$.

\textbf{Infinite-width training and SVM.} In the following, we focus on binary node classification with $y_i \in \{\pm 1\}$ and refer to \Cref{app:multi_class} for the multi-class case. In our learning setup, we follow \citet{chen2021equivalence} and \citet{gosch2024provable} and learn the parameters $\theta$ by optimizing the soft-margin loss:%, i.e., regularized hinge loss %by (sub)gradient descent 
\begin{align}
    \min_\theta \mathcal{L}(\theta,\rvy) = \min_\theta \frac{1}{2} \lVert \rmW^{(L+1)} \rVert^2_2 + C \sum_{i=1}^{m} \max(0 ,1-y_i f_\theta(\mG)_i)
    \label{eq:nn_loss}
\end{align}
where $C > 0$ is a regularization constant.
In the infinite-width limit, solving \Cref{eq:nn_loss} by (sub)gradient descent is equivalent to solving the dual problem of an SVM\footnote{Following previous works, we do not include a bias term.} with the NTK of $f_\theta(\mG)$ as its kernel:
\begin{align}
     \dual(\rvy):\ \min_{\rvalpha} - \sum_{i=1}^m \alpha_i + \dfrac{1}{2} \sum_{i=1}^m \sum_{j=1}^m y_i y_j \alpha_i \alpha_j \Theta_{i j} \,\, \text{s.t.} \,\, 0 \leq \alpha_i \leq C \,\, \forall i \in [m] 
     \label{eq:svm_dual}
\end{align}
where $\rvalpha \in \mathbb{R}^m$ are the SVM dual variables. % and the NTK %$\mTheta \in \mathbb{R}^{m \times m}$ 
%values $Q_{ij}$ are computed between all labeled nodes $i,j\in[m]$. 
The solution to \Cref{eq:svm_dual} is not guaranteed to be unique; hence, we denote the set of $\valpha$ vectors solving $\dual(\rvy)$ by $\mathcal{S}(\rvy)$. Given any $\valpha$, an SVM predicts the label of a test node $t$ by computing $\sign(\sum_{i=1}^m y_i \alpha_i Q_{ti})$.
%As the prediction of the so obtained SVM equals the one of the GNN $f_\theta$ in the infinite width limit, a certificate for the SVM results in a certificate for 
%The prediction of the SVM for a test node $t$ using the dual is given by $f_\theta^{SVM}(\rvx_t) =\sum_{i=1}^m y_i \alpha_i^* \Theta_{ti}$ for any $\valpha^* \in \mathcal{S}(\rvy)$, where $\Theta_{ti}$ is the NTK between the test node $t$ and training node $i$. Using the prediction, the class is assigned for $\rvx_t$ as $\sign(f_\theta^{SVM}(\rvx_t))$.
%Furthermore, for finite-width networks, the difference of the output to the infinite network is bounded with probability $\mathcal{O}(\frac{\ln h}{\sqrt{h}})$ where $h$ is the smallest width of the network \citep{arora2019exact,liu2020linearity}. Therefore, our certificate holds with a high probability for finite-width sufficiently wide networks.
%Furthermore, we focus on studying different architectures such as MLP, GCN \citep{kipf2017semisupervised}, SGC \citep{wu2019simplifying}, (A)PPNP \citep{gasteiger2019predict}, Graph Isomorphism Network (GIN) \citep{xu2018powerful} and GraphSAGE \citep{hamilton2017inductive} and GNNs with skip-connections and provide their definitions in \Cref{app:architecture_def}.

==> sections/app_architectures.tex <==
\section{Architecture definitions} 
\label{app:architecture_def}
We consider GNNs as functions $f_\theta$ with (learnable) parameters $\theta\in \mathbb{R}^q$ and $L$ number of layers taking the graph $\mG=(\mS, \mX)$ as input and outputs a prediction for each node. We consider linear output layers with weights $\mW^{L+1}$ and denote by $f_\theta(\mG)_i \in \mathbb{R}^K$ the (unnormalized) logit output associated to node $i$. In the following, we formally define the (G)NNs such as MLP, GCN \citep{kipf2017semisupervised}, SGC \citep{wu2019simplifying} and (A)PPNP \citep{gasteiger2019predict} considered in our study.

\begin{definition}[MLP]\label{def:mlp}
    The $L$-layer Multi-Layer Perceptron is defined as $f_\theta(\mG)_i=f_\theta^{MLP}(\vx_i)=\mW^{L+1}\phi^{(L)}_\theta(\vx_i)$. With $\phi_\theta^{l}(\vx_i)=\sigma(\mW^{(l)}\phi_\theta^{(l-1)}(\vx_i)+\vb^{(l)})$ and $\phi_\theta^{(0)}(\vx_i)=\vx_i$. $\mW^{(l)}\in\mathbb{R}^{d_{l+1} \times d_{l}}$ and $\vb^{(l)}\in\mathbb{R}^{d_l}$ are the weights/biases of the $l$-th layer with $d_0=d$ and $d_{L+1}=K$. $\sigma(\cdot)$ is an element-wise activation function. If not mentioned otherwise, we choose $\sigma(z) = \text{ReLU}(z) = \max\{0, z\}$.
\end{definition}

\begin{definition}[GCN \& SGC]\label{def:gcn}
A Graph Convolution Network $f_\theta^{GCN}(\mG)$ \citep{kipf2017semisupervised} of depth $L$ is defined as $f_\theta(\mG) =  \phi_\theta^{(L+1)}(\mG)$ with $\phi_\theta^{(l)}(\mG) = \rmS \sigma(\phi_\theta^{(l-1)}(\mG))\mW^{(l)}$ and $\phi_\theta^{(1)}(\mG) = \rmS\rmX\rmW^{(1)}$.
$\rmW^{(l)} \in \mathbb{R}^{d_{l-1} \times d_{l}}$ are the $l$-th layer weights, $d_{0} = d$, $d_{L+1} = K$, and %the element-wise activation function 
$\sigma(z)= \text{ReLU}(z)$ applied element-wise. A Simplified Graph Convolution Network $f_\theta^{SGC}(\mG)$ \citep{wu2019simplifying} is a GCN with linear %activation function 
$\sigma(z)= z$.
\end{definition}

%\begin{definition}[SGC]
%A Simplified Graph Convolution Network $f_\theta^{SGC}(\mG)$ \citep{wu2019simplifying} is a GCN with linear activation function 
%$\sigma(z)= z$.
%\end{definition}

\begin{definition}[(A)PPNP]\label{def:appnp}
The Personalized Propagation of Neural Predictions Network $f_\theta^{PPNP}(\mG)$ \citet{gasteiger2019predict} is defined as $f_\theta(\mG) = \rmP \rmH$ where $\rmH_{i,:} = f_\theta^{MLP}(\rvx_i)$ and $\rmP = \alpha(\rmI_{n} - (1-\alpha)\rmS)^{-1}$. The Approximate PPNP is defined with $\rmP = (1-\alpha)^K\rmS^K + \alpha \sum_{i=0}^{K-1} (1-\alpha)^i\rmS^i$ where $\alpha\in[0,1]$ and $K\in \mathbb{N}$ is a fixed constant.
\end{definition}

\label{sec_app:architecture_def}
Along with the GNNs presented in \Crefrange{def:mlp}{def:appnp}, we consider two variants of popular skip connections in GNNs as given a name in \citet{sabanayagam2023analysis}:
Skip-PC (pre-convolution), where the skip is added to the features before applying convolution \citep{kipf2017semisupervised}; 
and Skip-$\alpha$, which adds the features to each layer without convolving with $\rmS$ \citep{chenWHDL2020gcnii}.
To facilitate skip connections, we need to enforce constant layer size, that is, $d_i=d_{i-1}$.
Therefore, the input layer is transformed using a random matrix $\rmW$ to $\rmH_0 := \rmX \rmW $ of size $n \times h$ where $\rmW_{ij} \sim \mathcal{N}(0,1)$ and $h$ is the hidden layer size. 
Let $\rmH_i$ be the output of layer $i$  using which we formally define the skip connections as follows.

\begin{definition}[Skip-PC]
\label{def:pc}
In a Skip-PC (pre-convolution) network, the transformed input $\rmH_0$ is added to the hidden layers before applying the graph convolution $\rmS$, that is, $\forall i \in [L],
\phi_\theta^{(l)}(\mG) = \rmS \lp \sigma(\phi_\theta^{(l-1)}(\mG)) + \sigma_s \lp \rmH_0 \rp \rp \mW^{(l)}, $
% \rmH_i := \sqrt{\frac{c_\sigma}{h}} \rmS \lp \rmH_{i-1} + \sigma_s \lp \rmH_0 \rp\rp \rmW_{i}$, 
where $\sigma_s(z)$ can be linear or ReLU.
\end{definition}
Skip-PC definition deviates from \citet{kipf2017semisupervised} because we skip to the input layer instead of the previous one.
We define Skip-$\alpha$ as defined in \citet{sabanayagam2023analysis} similar to \citet{chenWHDL2020gcnii}.

\begin{definition}[Skip-$\alpha$] 
\label{def:alp}
Given an interpolation coefficient $\alpha\in(0,1)$, a Skip-$\alpha$  network is defined such that the transformed input $\rmH_0$ and the hidden layer are interpolated linearly, that is, 
$\phi_\theta^{(l)}(\mG) =  \lp \lp 1-\alpha \rp \rmS \phi_\theta^{(l-1)}(\mG) + \alpha \sigma_s \lp \rmH_0 \rp\rp \rmW_{i} ~\forall i \in [L]$, where $\sigma_s(z)$ can be linear or ReLU.
\end{definition}

